Synopsis: Secure and private trend inference from encrypted semantic embeddings

WhatsApp and many other commonly used communication platforms guarantee end-to-end encryption (E2EE), which requires that service providers lack the cryptographic keys to read communications on their own platforms. WhatsApp's privacy-preserving design makes it difficult to study important phenomena like the spread of misinformation or political messaging, as users have a clear expectation and desire for privacy and little incentive to forfeit that privacy in the process of handing over raw data to researchers, journalists, or other parties. We introduce Synopsis, a secure architecture for analyzing messaging trends in consensually-donated E2EE messages using message embeddings. Since the goal of this system is investigative journalism workflows, Synopsis must facilitate both exploratory and targeted analyses -- a challenge for systems using differential privacy (DP), and, for different reasons, a challenge for private computation approaches based on cryptography. To meet these challenges, we combine techniques from the local and central DP models and wrap the system in malicious-secure multi-party computation to ensure the DP query architecture is the only way to access messages, preventing any party from directly viewing stored message embeddings. Evaluations on a dataset of Hindi-language WhatsApp messages (34,024 messages represented as 500-dimensional embeddings) demonstrate the efficiency and accuracy of our approach. Queries on this data run in about 30 seconds, and the accuracy of the fine-grained interface exceeds 94% on benchmark tasks.

==> tikz/database.tex <==
\makeatletter
\tikzset{
    database/.style={
        path picture={
            \draw (0, 1.5*\database@segmentheight) circle [x radius=\database@radius,y radius=\database@aspectratio*\database@radius];
            \draw (-\database@radius, 0.5*\database@segmentheight) arc [start angle=180,end angle=360,x radius=\database@radius, y radius=\database@aspectratio*\database@radius];
            \draw (-\database@radius,-0.5*\database@segmentheight) arc [start angle=180,end angle=360,x radius=\database@radius, y radius=\database@aspectratio*\database@radius];
            \draw (-\database@radius,1.5*\database@segmentheight) -- ++(0,-3*\database@segmentheight) arc [start angle=180,end angle=360,x radius=\database@radius, y radius=\database@aspectratio*\database@radius] -- ++(0,3*\database@segmentheight);
        },
        minimum width=2*\database@radius + \pgflinewidth,
        minimum height=3*\database@segmentheight + 2*\database@aspectratio*\database@radius + \pgflinewidth,
    },
    database segment height/.store in=\database@segmentheight,
    database radius/.store in=\database@radius,
    database aspect ratio/.store in=\database@aspectratio,
    database segment height=0.1cm,
    database radius=0.25cm,
    database aspect ratio=0.35,
}
\makeatother

==> tikz/smartphone.tex <==
\makeatletter
\tikzset{
    smartphone/.style={
        path picture={
            \draw[rounded corners=\smartphone@roundedcorners, fill=black] (0,0) rectangle (\smartphone@width,\smartphone@height) {};
            \draw[fill=white] (\smartphone@screenoffset,{\smartphone@screenoffset*2}) rectangle ({\smartphone@width-\smartphone@screenoffset},{\smartphone@height-\smartphone@screenoffset}) {};
            \draw[fill=white] ({\smartphone@width/2}, \smartphone@screenoffset) circle ({\smartphone@screenoffset/2}) {};
            },
        minimum width=2*\smartphone@width + \pgflinewidth,
        minimum height=3*\smartphone@height + \pgflinewidth,
    },
    smartphone height/.store in=\smartphone@height,
    smartphone width/.store in=\smartphone@width,
    smartphone screen offset/.store in=\smartphone@screenoffset,
    smartphone rounded corners/.store in=\smartphone@roundedcorners,
    smartphone height=0.7cm,
    smartphone width=0.4cm,
    smartphone screen offset=0.08cm,
    smartphone rounded corners=3pt,
}
\makeatother

